Hypothesis Testing for Class-Conditional Label Noise

In this paper we provide machine learning practitioners with tools to answer the question: is there class-conditional noise in my labels? In particular, we present hypothesis tests to check whether a given dataset of instance-label pairs has been corrupted with class-conditional label noise, as opposed to uniform label noise, with the former biasing learning, while the latter -- under mild conditions -- does not. The outcome of these tests can then be used in conjunction with other information to assess further steps. While previous works explore the direct estimation of the noise rates, this is known to be hard in practice and does not offer a real understanding of how trustworthy the estimates are. These methods typically require anchor points -- examples whose true posterior is either 0 or 1. Differently, in this paper we assume we have access to a set of anchor points whose true posterior is approximately 1/2. The proposed hypothesis tests are built upon the asymptotic properties of Maximum Likelihood Estimators for Logistic Regression models. We establish the main properties of the tests, including a theoretical and empirical analysis of the dependence of the power on the test on the training sample size, the number of anchor points, the difference of the noise rates and the use of relaxed anchors.

==> reviews/uai2021.tex <==
R1,2 - Relevance of problem statement & workflow 

 Class-conditional label noise (CCN) has been shown to bias learning algorithms, as opposed to uniform label noise (UN). Therefore, undetected CCN in a dataset will render conclusions drawn from a model invalid. Our test is designed to be performed after data collection and annotation to offer a quality measure wrt label noise. If the test is positive, then the practitioner could resort to (1) a modified data labelling procedure (e.g., active learning in the presence of noise), (2) seek methods to make their training robust (e.g., algorithms for learning from noisy labels), or (3) drop the dataset altogether. 

R1,2 - CCN vs Instance-Dependent Noise (IDN) 

UN is the most basic scenario where learning can be unbiased under mild conditions. The next step is CCN, where learning is in general biased. A motivating example of CCN is given in Frénay and Verleysen [2013] in the form of medical case-control studies, where different tests may be used for subject and control. IDN is a further generalisation where the probability of label flipping is allowed to depend on the features. This is the first work to introduce principled quality check on the labels of a dataset and it could serve as a starting point to devise tests of IDN as well. One potential way of extending our framework to test for IDN could be to have anchor points at different contours, i.e., 0.20, 0.30, ... 0.70. 

R1,2,4 - Access to anchor-points 

As in related works, anchor-points need to be provided by the experts. The field of probability elicitation is not new and is relevant to Bayesian statistics, where prior knowledge comes to aid information extracted from data. In the case of relaxed anchors, the practitioner does not need to know $\delta$. In our analysis we show the dependence of the test on it, theoretically and empirically.  

Re Def. 2.4: we define relaxed anchors that are not necessarily equal to 0.50 but are close to it. We model this closeness with an added uniform rv. This is how we model the expert picking a (relaxed) anchor - a point close to the 0.50 contour. 

R1 - Real data study 

Our aim in this work is to draw attention over this scenario, propose a theoretically grounded procedure and analyse its properties. We wish to present real world case study in separate work. 

R5 - Fisher (RF) and Neyman-Pearson (NP) 

The reviewer is right in saying that our analysis is more in-line with framework given by NP. We are not claiming that p-values are error probabilities - in our experiments we present aggregate p-values (from separate runs) simply as a means of displaying differences between different configurations. This is a very useful comment, and we will clarify this in the text. 

R1 - MLE performance under CCN  

We are not aware of results quantifying how poorly the MLE would perform under CCN, beyond being biased. Wrt robustifying against label noise the following reference could be of relevant: "Does label smoothing mitigate label noise?" by Michal Lukasik et al. 

 

Specific points: 

R2:  

“It seems the test proposed is just whether the unknown parameter beta_0 in a logistic model belongs to a certain subspace; why does rejecting this null indicates CCN?” 

We refer the reviewer to Eqs.5-7 and accompanying text that show why rejecting the null suggests the presence of CCN.  

Logistic loss -> $\Psi(f) + \Psi(-f) = K.$ 

Eq.4 of Ghosh et al. [2015] 

““This fails in the case $\eta(x) \in \{0,1\}$.” ...” 

This has to do with the anchor being of this form, i.e. an anchor point with a known posterior of either 0 or 1. 

On Eq.7: 

Under the null: 

\tilde{\eta} = (1-\tau)\eta + \tau(1-\eta) 

\tilde{\eta}(1-\tilde{\eta}) = (1-2\tau)^2\eta(1-\eta) + \tau(1-\tau) 

now we let: \eta=1/2 and get: 

1/4(1-2\tau)^2 + \tau(1-\tau) = 1/4 

which when squared gives: 1/16 

Eq.2 shows how the data generating process is affected by CCN. 

On the power computation in Eq.12: 

In Eq.12 we are not presenting the expectation of the fraction $\frac{b_k}{b_1}$ but rather just substitute $v$ with its expectation to better understand the relationship. 

On Eq.13: 

By the law of total variance, we have the 'expectation of the variance' term which we use in Eq.13, and the 'variance of the expectation' which we show in Eq.14. The second term is less significant and as we show goes away as we increase $k$. This will be clarified. 

"If the analyst knows certain points are anchor points, could he or she use this knowledge to get a better estimate of the unknown logistic regression parameter, and therefore enhance the power of the test..." 

Interesting direction -- one way could be to enforce them as constraints in a mathematical program formulation. The second part of the Q re the power of the test is unclear to us – we are already using anchor-points for the test. 

R5 

\pi = P(y=1) - the class prior. 

v(x) denotes the variance under the null, as opposed to having the tilde. 

On multiclass setting and multiple testing 

This is correct, adjustments should be made in accordance with multiple testing corrections. 

 

==> sections/case1.tex <==
% \subsection{Case \#1: we know $\pi$}
% \todo[inline]{consider moving to the appendix}
First we study the scenario where the user knows the true prior: $\pi$, has an observed $\hat{\pi} = \hat{\mathbb{P}}(\bar{y}=1)$ and wants to assess whether the data are contaminated with noise.
Our two-sided hypothesis test is as follows:
\begin{align*}
    & \mathcal{H}_{0}: \hat{\pi} = \pi \\
    & \mathcal{H}_{1}: \hat{\pi} \neq \pi
\end{align*}
This is a two-sided test.

For this there are:
\subsubsection{Binomial Hypothesis test}
\paragraph{Take 1 - Binomial Test}
$$
Bin(n, k, \pi_{0}) = \mathbb{P}(X=k)=\left(\begin{array}{l}
n \\
k
\end{array}\right) \pi_{0}^{k}(1-\pi_{0})^{n-k}
$$
$k=n\times\hat{\pi}_0$

\paragraph{Take 2 - Large Samples}
Large sample gaussian approximation
$z$-test
$$
Z=\frac{k-n \pi_0}{\sqrt{n \pi_0(1-\pi_0)}}
$$

\todo[inline]{For this we could do the calculations of power etc but probably no experiments}
% \subsubsection{Bayes Factor}
% \textrm{https://en.wikipedia.org/wiki/Bayes_factor}

==> sections/case2.tex <==
% \subsection{Case \#2: we have anchor points}
\todo[inline]{proper book references}
We are provided with dataset $(\boldsymbol{X},~\boldsymbol{y})$ with $\boldsymbol{X} \in \mathbb{R}^{n\times d}$ and $\boldsymbol{y} \in \{-1, 1\}^n$ and a set of anchor points $\mathcal{A}_{\sfrac{1}{2}}^k$.

We assume the feature vectors ($\boldsymbol{x}$) have been augmented with $ones$ such that we have $\boldsymbol{x} \to (1,~\boldsymbol{x})$. We also assume the following (correct) model:
\begin{equation}
y_{i} \sim \text {Bernouilli}\left(\eta_{i}\right), \quad \eta_{i}=\frac{1}{1+\exp \left(-\theta^T x_{i}\right)}, \quad \forall i \in [n]
\end{equation}

If we let:
\begin{equation}
\hat{\theta}_{n} := \underset{\theta \in \Theta}{\operatorname{argmax}}~\ell_n\left(\theta \mid D_n\right) = \underset{\theta \in \Theta}{\operatorname{argmax}}~\prod_{i=1}^n~\ell_i\left(\theta \mid x_i,~y_i\right)
\end{equation}
where: $l\left(\theta \mid x_i,~y_i\right) = y_i\log\eta_i + (1-y_i)\log(1-\eta_i)$.

Then under conditions [REF] we get:
\begin{equation}
\sqrt{n}\left(\hat{\theta}_{n}-\theta_{0}\right)~\stackrel{D}{\longrightarrow} \mathcal{N}\left(0,~I_{n}(\theta_0)\inv\right)
\end{equation}

where $I_{\theta_{0}}$ denotes the Fisher-Information Matrix defined as: 
\begin{equation}
I_{n}(\theta_0)=\mathbb{E}_{\theta}\left(-\frac{\partial^{2} \ell_{n}(\theta ; Y \mid x)}{\partial \theta \partial \theta^{\top}}\right)=\mathbb{E}_{\theta}\left(-H_{n}(\theta ; Y \mid x)\right)
\end{equation}
where the expectation is with respect to the conditional distribution, and $H_n$ denotes the Hessian matrix.

As important remark is that we can express $I_{n}(\theta_0) = n\cdot I_{i}(\theta_0)$, which shows that as $n \to \infty$, the variance of the MLE estimator goes to $0$.

With the use of the delta method [REF?] we can get an asymptotic distribution for the posterior:
\begin{equation}
    \sqrt{n}(\hat{\eta}(x)-\eta(x)) \stackrel{D}{\longrightarrow} \mathcal{N}\left(0,~[\eta(x)\{1-\eta(x)\}]^{2}\cdot x^{\top} I_{\theta_{0}}\inv x\right)
\end{equation}

This wouldn't work with $\eta(x) \in \{0,~1\}$, so we can only work with $\sfrac{1}{2}$. Which, together with the approximation of the Fisher-Information matrix with the empirical Hessian, we get:

\begin{equation}
    \hat{\eta}(x) \stackrel{D}{\longrightarrow} \mathcal{N}\left(\frac{1}{2},~\frac{1}{16}\cdot x^{\top} \hat{H}_n x\right)
\end{equation}
where $\hat{H}_n = (X^TDX)^\inv$, where $D$ is a diagonal matrix, with $D_{ii} = \sigma_i(1 - \sigma_i)$, where $\sigma_i = \sigma(x_i^T\hat{\beta})$.

\paragraph{What if $\alpha = \beta = \tau \neq 0?$}\\
Then we have:
\begin{equation*}
    \tilde{\eta}(x) = (1 - 2\tau)\cdot\eta(x) + \tau
\end{equation*}
which, when we plug in:~$\eta(x) = \sfrac{1}{2}$, we get:~$\tilde{\eta}(x) = \sfrac{1}{2}$

This allows us to formulate our hypothesis test as follows:
\begin{align*}
    & \mathcal{H}_{0}: \alpha = \beta \\
    & \mathcal{H}_{1}: \alpha \neq \beta \\
\end{align*}

Where we have:
\begin{align*}
    &~\mathcal{H}_{0}: \hat{\eta}(x) \sim \mathcal{N}\left(\frac{1}{2},~\frac{1}{16}\cdot x^{\top} \hat{H} x\right) = \mathcal{N}\left(\frac{1}{2},~v(x)\right)\\
    &~\mathcal{H}_{1}: \hat{\eta}(x) \sim \mathcal{N}\left(\frac{1-\alpha+\beta}{2},~\frac{[(1-\alpha+\beta)(\beta-\alpha)]^2}{16}\cdot x^{\top} \hat{\tilde{H}} x\right) = \mathcal{N}\left(\frac{1+\alpha-\beta}{2},~\tilde{v}(x)\right)\\
\end{align*}
\paragraph{Statistical Significance and Power of the test:}
\begin{equation*}
    \textrm{Significance:}~~a = \mathbb{P}(\textrm{reject}~ \mathcal{H}_0~|~\mathcal{H}_0~\textrm{is True})
\end{equation*}
\begin{equation*}
    \frac{\hat{\eta}(x) - \sfrac{1}{2}}{\sqrt{v(x)}} \sim \mathcal{N}(0, 1)\\
\end{equation*}
Retain $\mathcal{H}_0$ if:
\begin{align*}
    &~z_{\sfrac{a}{2}} \leq \frac{\hat{\eta}(x) - \sfrac{1}{2}}{\sqrt{v(x)}} \leq z_{1-\sfrac{a}{2}}\\
    &~-z_{1-\sfrac{a}{2}} \leq \frac{\hat{\eta}(x) - \sfrac{1}{2}}{\sqrt{v(x)}} \leq z_{1-\sfrac{a}{2}}\\
    &~-z \leq \frac{\hat{\eta}(x) - \sfrac{1}{2}}{\sqrt{v(x)}} \leq z\\
    &~-z\cdot \sqrt{v(x)} + \sfrac{1}{2} \leq \hat{\eta}(x) \leq z\cdot\sqrt{v(x)} + \sfrac{1}{2}\\
    &~L_1 \leq \hat{\eta}(x) \leq U_1 \\
\end{align*}
Power:~~1 - $b_1$ = $\mathbb{P}(\textrm{reject}~ \mathcal{H}_0~|~\mathcal{H}_0~\textrm{is False})$
\begin{align*}
    b_1&~=\mathbb{P}(\textrm{retain}~ \mathcal{H}_0~|~\mathcal{H}_0~\textrm{is False})\\
    &~=\mathbb{P}(L_1 \leq \hat{\eta}(x) \leq U_1~|~\hat{\eta}(x) \sim \mathcal{N}\left(\frac{1+\alpha-\beta}{2},~\tilde{v}(x)\right))\\
    &~=\mathbb{P}(L_1 \leq \hat{\eta}(x) \leq U_1~|~\hat{\eta}(x) = \frac{1+\alpha-\beta}{2} + \sqrt{\tilde{v}(x)}\cdot\epsilon)\\
    &~=\mathbb{P}(\frac{L_1 - \sfrac{1+\alpha-\beta}{2}}{\sqrt{\tilde{v}(x)}}~\leq~\epsilon~\leq~\frac{U_1 - \sfrac{1+\alpha-\beta}{2}}{\sqrt{\tilde{v}(x)}})\\
    &~=\mathbb{P}(\frac{-z\cdot\sqrt{v(x)} + h}{\sqrt{\tilde{v}(x)}}~\leq~\epsilon~\leq~\frac{z\cdot\sqrt{v(x)} + h}{\sqrt{\tilde{v}(x)}})\\
    &~=\Phi(\frac{z\cdot\sqrt{v(x)} + h}{\sqrt{\tilde{v}(x)}}) - \Phi(\frac{-z\cdot\sqrt{v(x)} + h}{\sqrt{\tilde{v}(x)}})\\
    % &~=\Phi(\frac{z\cdot\sqrt{v(x)} + \frac{\beta-\alpha}{2}}{\sqrt{\tilde{v}(x)}}) - \Phi(\frac{-z\cdot\sqrt{v(x)} + \frac{\beta-\alpha}{2}}{\sqrt{\tilde{v}(x)}})
\end{align*}
where we have used: $h = \frac{\beta-\alpha}{2}$, for ease of notation.

% \paragraph{How do $v(x)$ and $\tilde{v}(x)$ differ?}\\
% A worst case analysis gives the following:
% \begin{equation*}
%     \max_{z\in\mathbb{R}^d}\frac{z^T(X^T\tilde{D}X)\inv z}{z^T(X^TDX)\inv z}=\max_{z\in\mathbb{R}^d}\frac{z^TX^TDXz}{z^TX^T\tilde{D}Xz}=\max_{p\in\mathbb{R}^d}\frac{p^TDp}{p^T\tilde{D}p}=\max_{p\in\mathbb{R}^d}\frac{w^TD\tilde{D}\inv w}{w^Tw}
% \end{equation*}
% where the last maximisation equals the largest eigenvalue of the product: $\lambda_{max}(D\tilde{D})$, which in turn equals: $\max_{\boldsymbol{x} \in \boldsymbol{X}}\frac{\eta(\boldsymbol{x})(1-\eta(\boldsymbol{x})}{\tilde{\eta}(\boldsymbol{x})(1-\tilde{\eta}(\boldsymbol{x})}$. 

\paragraph{What if we have Multiple Anchors?}\\

The following expectation ($\mathbb{E}$), and variance ($\mathbb{V}$) operators, unless specified otherwise, are with respect to randomness in $\hat{\theta}_{mle}$.

\begin{align*}
    & \mathbb{E}\hat{\eta} = \sfrac{1}{2} \\
    & \mathbb{V}\hat{\eta} = [\eta(1-\eta)]^2\cdot x^THx \\
    & \mathbb{E}[\frac{1}{k}\sum_{i=1}^k\hat{\eta}_i] = \sfrac{1}{2} \\
    & \mathbb{V}[\frac{1}{k}\sum_{i=1}^k\hat{\eta}_i] = \frac{1}{k^2}\left[\sum_{i=1}^k \mathbb{V}\hat{\eta}_i + 2\cdot\sum_{i, j>i} Cov(\hat{\eta}_i, \hat{\eta}_j) \right] \\
    & \textrm{let}~\gamma_i = \hat{\eta}_i(1-\hat{\eta}_i)\\
    & Cov(\hat{\eta}_i, \hat{\eta}_j) = \gamma_i\gamma_j\cdot x_i^THx_j ~~~~\left[\textrm{See Section}~\ref{appendix:covariance}\right]\\
    & \mathbb{V}[\frac{1}{k}\sum_{i=1}^k\hat{\eta}_i] = \frac{1}{16}\cdot \bar{x}^TH\bar{x}
\end{align*}

\paragraph{What if the anchors are random?}\\

If we have $\boldsymbol{x}$ such that $\eta(\boldsymbol{x}) = \sfrac{1}{2}$, it implies that $\boldsymbol{x}^T\beta_0 = 0$, so that for an orthonormal basis $\boldsymbol{U}$, $\boldsymbol{x} = \boldsymbol{U}\boldsymbol{r}$. Without loss of generalisation we let $\boldsymbol{U}_{:,0} = \frac{\beta_0}{\|\beta_0\|_{2}}$, and therefore $\eta(x) = \sfrac{1}{2} \to \boldsymbol{r}_0 = 0$. In words: $\forall \boldsymbol{x} \in \mathcal{A}$ we have that $\boldsymbol{x}$'s component in the direction of $\beta_0$ is $0$.

Now we make the assumption that $\boldsymbol{x}$'s are random with $r_j \sim \mathbb{U}([-c,~c])$. Therefore, $\mathbb{E}r_j = 0$, and $\mathbb{V}r_j = \frac{c^2}{3}$. In the following we use the subscript $S$ in the operator $\mathbb{E}_{S}$ to denote the randomness in choosing the set $\mathcal{A}$.

Combining these we get:
\begin{equation*}
    \mathbb{E}_{S} x^THx = \mathbb{E}_{S} r^TUHU^Tr = \frac{dc^2}{3}\cdot tr(UHU^T) = \frac{dc^2q}{3}
\end{equation*}
where $q=tr(H)$.

While for $k$ anchor points chosen independently at random, we get:
\begin{equation*}
    \mathbb{E}_{S}[\frac{1}{k^2}\sum_{i,j}^kx_i^THx_j] = \mathbb{E}_{S} \frac{1}{k^2}\sum_{i,j}^k r_i^TUHU^Tr_j = \frac{dc^2}{3k}\cdot tr(UHU^T) = \frac{dc^2q}{3k}
\end{equation*}


Following the same derivation as above [REF] we get:
\begin{equation*}
    b_k = \Phi(\frac{z\cdot\sqrt{v(\bar{x})} + \frac{\beta-\alpha}{2}}{\sqrt{\tilde{v}(\bar{x})}}) - \Phi(\frac{-z\cdot\sqrt{v(\bar{x})} + \frac{\beta-\alpha}{2}}{\sqrt{\tilde{v}(\bar{x})}})
\end{equation*}

If we let $v = \mathbb{E}_Sv(x)$ (similarly $\tilde{v} = \mathbb{E}_S\tilde{v}(x)$), then we have seen that $\mathbb{E}_Sv(\bar{x}) = \frac{v}{k}$ (Reminder: expectations are with respect to the randomness in picking the anchor-points). Then we have:
\begin{equation}
    \frac{b_k}{b_1} = \frac{\Phi(\frac{z\sqrt{v} + h\sqrt{k}}{\sqrt{\tilde{v}}}) - \Phi(\frac{-z\sqrt{v} + h \sqrt{k}}{\sqrt{\tilde{v}}})}{\Phi(\frac{z\sqrt{v} + h}{\sqrt{\tilde{v}}}) - \Phi(\frac{-z\sqrt{v} + h}{\sqrt{\tilde{v}}})} \leq 1
\end{equation}

\todo[inline]{my attempt at comparing them is the figure below...}
\begin{figure}[ht]
    \centering
    \includegraphics[scale=0.30]{figures/power_and_k.pdf}
    \caption{Power of the hypothesis test as a function of $\beta-\alpha$, for a range of different $k$s. We set $v = \sfrac{1}{16}\cdot(X^TDX)\inv = 0.1$.}
\end{figure}
 
 
\subsection{Relaxed Anchors}
Let $x$ be such that $\eta(x) = \frac{1}{2} + \epsilon$, where $\epsilon \in [-\delta, \delta]$ with $\delta \ll 1$.
\begin{align*}
    & \mathbb{E}\hat{\eta} = \sfrac{1}{2} + \epsilon \\
    & \mathbb{E}_{S}\mathbb{E}\hat{\eta} = \sfrac{1}{2} \\
    & [\eta(1-\eta)]^2 \rightarrow [(\frac{1}{2} + \epsilon)(\frac{1}{2} - \epsilon)]^2 = [\frac{1}{4} - \epsilon^2]^2 \approx \frac{1}{16} \\
    & \mathbb{V}\hat{\eta} = [\eta(1-\eta)]^2\cdot x^THx \\
    & \mathbb{E}\frac{1}{k}\sum_{i=1}^k\hat{\eta}_i = \sfrac{1}{2} \\
    & \mathbb{V}\frac{1}{k}\sum_{i=1}^k\hat{\eta}_i = \frac{1}{k^2}\left[\sum_{i=1}^k \mathbb{V}\hat{\eta}_i + 2\cdot\sum_{i, j>i} Cov(\hat{\eta}_i, \hat{\eta}_j) \right] \\
    & \textrm{let}~\gamma_i = \hat{\eta}_i(1-\hat{\eta}_i)\\
    & Cov(\hat{\eta}_i, \hat{\eta}_j) = \gamma_i\gamma_j\cdot x_i^THx_j\\
    & \mathbb{V}\frac{1}{k}\sum_{i=1}^k\hat{\eta}_i = \frac{1}{16}\cdot \bar{x}^TH\bar{x}
\end{align*}


==> sections/checklist.tex <==
\section{Checklist}

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{Section 3.5}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerTODO{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerTODO{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{}
	\item Did you include complete proofs of all theoretical results?
    \answerYes{}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerNo{not significant}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerNA{}
  \item Did you mention the license of the assets?
    \answerNA{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{google drive anonymised link}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}

==> sections/notes.tex <==
\section{Notes}
\begin{enumerate}
    \item We cannot tell whether there is uniform noise: $\alpha=\beta$.
    \item We can only identify the term $\beta - \alpha$.
    \item We could average over $k$ anchor points, and get a $1/k$ term in the variance.
    \item We could allow for $\eta(x) + \epsilon$, where $\epsilon \in [-u, u]$, with $u$ being something small, i.e. $0.10$. and with $\mathbb{E}e = 0$. This would imply an unbiased mean of the distribution ($f$), but we would end up overestimating the variance - but by a factor proportional to $\frac{\hat{\mathbb{E}}\epsilon^2}{2}$.
\end{enumerate}

The idea is to use to these equations to have a hypothesis test for $\alpha$ and $\beta$. 
Problems:
\begin{enumerate}
    \item Would be nice to have similar results with a richer model class such as Gaussian Process Classification
    \item How does this change when the user provides us with $k$ anchor points? This would mean that now our test would depend on both the sample size and the number of anchor points. -- SOLVED, I think
    \item A baseline would be knowing the true class priors, and carrying out hypothesis test for the observed priors.
\end{enumerate}
